Estimating Rank-One Spikes from Heavy-Tailed Noise via Self-Avoiding Walks

We study symmetric spiked matrix models with respect to a general class of noise distributions. Given a rank-1 deformation of a random noise matrix, whose entries are independently distributed with zero mean and unit variance, the goal is to estimate the rank-1 part. For the case of Gaussian noise, the top eigenvector of the given matrix is a widely-studied estimator known to achieve optimal statistical guarantees, e.g., in the sense of the celebrated BBP phase transition. However, this estimator can fail completely for heavy-tailed noise. In this work, we exhibit an estimator that works for heavy-tailed noise up to the BBP threshold that is optimal even for Gaussian noise. We give a non-asymptotic analysis of our estimator which relies only on the variance of each entry remaining constant as the size of the matrix grows: higher moments may grow arbitrarily fast or even fail to exist. Previously, it was only known how to achieve these guarantees if higher-order moments of the noises are bounded by a constant independent of the size of the matrix. Our estimator can be evaluated in polynomial time by counting self-avoiding walks via a color -coding technique. Moreover, we extend our estimator to spiked tensor models and establish analogous results.

==> GaussianAlgorithm.tex <==

%  Obsolete
% ************




% \section{Algorithm for partial observation spiked tensor model with Gaussian noise}\label{nonMultilinear}
% From discussion before we note that in partial observation case the above distribution independent algorithm succeeds when $\frac{m}{n^3}\lambda^2 n^{3/2}\ell^{1/2}=\omega(1)$. However, low degree method predicts that when $m\lambda^4=\omega(1)$ polynomial time algorithm exists. We will show that very simple algorithm exists in this case
% % \algorithmstyle{ruled}
% % \begin{algorithm}[H]
% %  \KwData{Entry locations $\Omega\subseteq [n]^{\otimes 3}$ and corresponding values $\{Y_{ijk} : (i,j,k)\in\Omega\}$ sampled from $\mathbb{P}$ or $\mathbb{Q}$}
% %  \KwResult{The distribution from which $Y$ is sampled}
% %   \eIf{thresholding polynomial $P_\Omega(Y)=\Omega(m\lambda^2)$}{
% %   return spiked tensor model\;
% %   }{
% %   return Gaussian model\;
% %   }
% %   \caption{Strong detection algorithm for Gaussian noise}
% % \end{algorithm}

% \begin{theorem}
% If the spiked prior $x\sim \mathsf{Rademacher}\{\pm 1\}$, the algorithm thresholding $P(Y)$ will distinguish the null distribution and planted distribution with probability
%     $$1-6\exp{\left(-\frac{m}{3}\right)}-4\exp{\left(-\frac{m\lambda^2}{8}\right)}-\exp{\left(-\frac{m\lambda^4}{2}\right)}$$.
%     Therefore, it succeeds in strong detection when  $m\lambda^4=\omega(1)$ and $m\gg 1$
% \end{theorem}
% \begin{proof}
%     Under measure $\mathbb{Q}$ because $P_{\Omega}(Y)$ is Hermite polynomial, we have
%     \begin{equation*}
%         \E_{\mathbb{Q}} P_\Omega(Y)=0
%     \end{equation*}
%     and
%     \begin{equation*} P_\Omega(Y)=\sum_{(i,j,k)} \mathbf{1}_{(i,j,k)\in\Omega} (W_{ijk}^2-1)
%     \end{equation*}
%     where $W_{ijk}\sim N(0,1)$ and  $\mathbf{1}_{(i,j,k)\in\Omega}\sim \mathsf{Bern}(m/n^3)$.
%     Conditioning on $\Omega$, we have
%     \begin{equation*}
%         \mathbb{Q}\left[\left\lvert\sum_{(i,j,k)\in\Omega} (Y_{ijk}^2-1)\right\rvert \geq t\right]\leq 2\exp{\left(- \frac{t^2}{8\lvert\Omega\rvert}\right)}\quad \forall t<1
%     \end{equation*}
%     By Chernoff bound we have
%     \begin{equation*}
%       \lvert\Omega\rvert=\sum_{(i,j,k)} \mathbf{1}_{(i,j,k)\in\Omega}=m(1\pm \delta)
%     \end{equation*}
%     with probability $1-2\exp{\left(-\frac{m\delta^2}{3}\right)}$. Therefore by union bound, with probability $1-2\exp{(-\frac{m}{3})}-2\exp{(-\frac{t^2}{16})}$ we have
%     $P_\Omega(Y)<t\sqrt{m}$.
    
%     Second we analyze $P_\Omega(Y)$ under measure $\mathbb{P}$. In this case, we have
%     \begin{equation*}
%         \sum_{(i,j,k)\in\Omega}(Y_{ijk}^2-1)=\sum_{(i,j,k)\in\Omega} (\lambda^2+2\lambda x_ix_jx_kW_{ijk})+\sum_{(i,j,k)\in\Omega}(W_{ijk}^2-1)
%     \end{equation*}
%     For $\sum_{(i,j,k)\in\Omega}(W_{ijk}^2-1)$, this is the same as $P_\Omega(Y)$ in measure $\mathbb{Q}$ and is upper bounded by $t\sqrt{m}$ with probability $1-2\exp{\left(-\frac{m}{3}\right)-2\exp{\left(-\frac{t^2}{16}\right)}}$. On the other hand, $$\sum_{(i,j,k)\in\Omega}\lambda^2=\Omega(\lambda^2 m)$$ with probability $1-\exp{\left(-\frac{m}{3}\right)}$ by Chernoff bound. Further we have 
%     \begin{equation*}
%         \sum_{(i,j,k)\in\Omega}2\lambda x_ix_jx_k W_{ijk}
%         =2\lambda \sum_{(i,j,k)\in\Omega} W^{\prime}_{ijk}
%     \end{equation*}
%     where $W^{\prime}_{ijk}$ is also i.i.d sampled from $N(0,1)$. By Hoeffding bounds, we have
%         $$
%         \left\lvert2\lambda \sum_{(i,j,k)\in\Omega} W^{\prime}_{ijk}\right\rvert\leq
%         2\lambda |\Omega|^{1/2} \delta
%         $$ 
%         with probability $1-2\exp{\left(-\frac{\delta^2}{2}\right)}$. As before we have $|\Omega|<2m$ with probability $1-\exp{\left(-\frac{m}{3}\right)}$. By union bound, $$ 
%          \left\lvert\sum_{(i,j,k)\in\Omega}2\lambda x_ix_jx_k W_{ijk}\right\rvert
%          \leq 4\lambda m^{1/2} \delta
%         $$ 
%         with probability $1-\exp{\left(-\frac{m}{3}\right)}-2\exp{\left(-\frac{\delta^2}{2}\right)}$. 
        
%         In all by union bound, with probability $1-6\exp{\left(-\frac{m}{3}\right)}-4\exp{\left(-\frac{t^2}{16}\right)}-\exp{\left(-\frac{\delta^2}{2}\right)}$, we have
%         \begin{equation*}
%          P_\Omega(Y)=\Omega(m\lambda^2-2\sqrt{m} \lambda \delta-t\sqrt{m})
%         \end{equation*}
%         For $m\lambda^4=\omega(1)$,$\delta=o(\sqrt{m\lambda^2})$ and $t=o(\sqrt{m\lambda^4})$, this implies $P_\Omega(Y)=\Omega( m\lambda^2)=\omega(t\sqrt{m})$. Therefore taking $\delta$ as $o(\sqrt{m\lambda^2})$ and $t$ as $o(\sqrt{m\lambda^4})$,  thresholding $P_\Omega(Y)$ at $\Omega(m\lambda^2)$, we get an algorithm distinguishing planted distribution $\mathbb{P}$ and null distribution $\mathbb{Q}$ with probability $1-6\exp{\left(-\frac{m}{3}\right)}-4\exp{\left(-\frac{m\lambda^2}{8}\right)}-\exp{\left(-\frac{m\lambda^4}{2}\right)}$
% \end{proof}

==> LowDegreeStrongDetection.tex <==
\subsection{Low degree strong  detection algorithm}
\begin{definition}[Strong detection in general spiked Wigner model]\label{defDetectionSpikedMatrix}
For general spiked Wigner model, we have  $Y=\lambda xx^\top+W$,we want to distinguish two families of distribution:
\begin{itemize}
    \item planted distribution $\mathbb{P}$: where $Y$ is sampled from spiked Wigner model with $\lambda=\bar{\lambda}$
    \item null distribution $\mathbb{Q}$: where $Y$ is sampled with $\lambda=0$
\end{itemize}
\end{definition}

\begin{definition}[Strong detection in general spiked tensor model]\label{defDetectionSpikedTensor}
   In general spiked tensor model $Y=\lambda \mathbf{x}^{\otimes p}+W$,  we want to distinguish two families of distributions
    \begin{itemize}
        \item planted distribution $\mathbb{P}$ where $Y$ sampled from spiked tensor model with  $\lambda=\bar{\lambda}$
        \item null distribution $\mathbb{Q}$ where entries in   $Y$ are sampled with $\lambda=0$
    \end{itemize}
    For strong and weak recovery as defined above, given tensor $Y$ we estimate the hidden vector $x$
\end{definition}

\begin{definition}[Strong detection]
Strong detection here means that we can distinguish two distributions with high probability. This is to say, given matrix/tensor $Y$ sampled from planted distribution $\mathbb{P}$ and null distribution $\mathbb{Q}$ with equal probability, we need to find a function of entries in $Y$: $f(Y)\in\{0,1\}$ such that
\begin{equation*}
    \frac{1}{2}\mathbb{P}[f(Y)=1]+\frac{1}{2}\mathbb{Q}[f(Y)=0]=1-o(1)
\end{equation*}
\end{definition}
It's not explicitly stated  in previous literature how to obtain strong detection algorithm via low degree method. The following self-clear fact provides a systematic way for doing so. 
\begin{theorem}[Low degree polynomial thresholding algorithm]
 Given $Y$ sampled from $\mathbb{P}$ and $\mathbb{Q}$ with equal probability, For  polynomial $P(Y)=\sum_{\alpha\in S_\ell}\hat{\mu}_\alpha\chi_\alpha(Y)$ where $\{\chi_\alpha(Y):\alpha \in S_\ell\}$ is a set of  polynomial basis orthonormal under measure $\mathbb{Q}$ and $\hat{\mu}_\alpha$ is the Fourier coefficient of likelihood ratio between planted and null distribution $\mu(Y)=\frac{\mathbb{P}(Y)}{\mathbb{Q}(Y)}$ corresponding to basis $\chi_\alpha(Y)$: $\hat{\mu}_\alpha=\E_{\mathbb{P}} \chi_\alpha(Y)$, if we have diverged low degree likelihood ratio $\sum_{\alpha\in S_\ell} \hat{\mu}_\alpha^2 =\omega(1)$ and concentration property $\E_{\mathbb{P}} P^2(Y)=(1+o(1)) \left(\E_{\mathbb{P}} P(Y)\right)^2$, then this implies strong detection algorithm by thresholding polynomial $P(Y)$. 
\end{theorem}
\begin{proof}
    Since $\sum_{\alpha\in S_\ell} \hat{\mu}_\alpha^2 =\omega(1)$, we have $\E_{\mathbb{P}} P(Y)=\E_{\mathbb{Q}} P^2(Y)=\omega(1)$. By Chebyshev's inequality, for $Y\sim \mathbb{P}$ w.h.p we have $P(Y)=(1\pm o(1)) \E_{\mathbb{P}} P(Y)=\omega(\sqrt{\E_{\mathbb{Q}} P^2(Y)})$ while for $Y\sim \mathbb{Q}$ w.h.p we have $P(Y)=O(\sqrt{\E_{\mathbb{Q}} P^2(Y)})$
\end{proof}

For strong detection we use the estimator based on cycle
\begin{definition}[Simple cycle estimator]\label{simCycleMatrix}
    We use the following thresholding polynomial $P(Y)=\sum_{\alpha\in \textrm{CYC}_{\ell}} \chi_\alpha(Y)$
    where $\textrm{CYC}_{\ell}$ denotes the set of simple cycle with length $\ell$ on $n$ vertices and $\chi_\alpha(Y)=\prod_{(v_1,v_2)\in \alpha} Y_{v_1,v_2}$    
\end{definition}

\begin{lemma}\label{matrixThresholding}
In strong detection problem of spiked matrix model defined in \ref{defSpikedMatrix}, for $\lambda n^{1/2}=\delta=1+\Omega(1)$,set $\ell=O(\log_{\delta}n)$, then in planted distribution $Y\sim \mathbb{P}$ we have $P(Y)$ in definition \ref{simCycleMatrix} is $\Omega(n^{\ell+1} \lambda^{\ell})$ with high probability. On the other hand, for null distribution $Y\sim \mathbb{Q}$,  we have $P(Y)=o(n^{\ell+1} \lambda^{\ell})$ with high probability. 
\end{lemma}
This implies strong detection algorithm by thresholding polynomial.


 

==> NonBacktracking.tex <==
\subsection{Non-Backtracking walk estimator} 
\Snote{I'm not sure I understand the purpose of this section. It seems like it just contains a result, rather than any proofs or technical arguments. If it is a result we want to highlight in the main version of the paper, we should put it in the contributions section, rather than buried here, I think.}

\begin{definition}[Non-backtracking walk estimator]
For matrix  $Y$ and constant $k$, we define  the associated $k$-step non-backtracking walk estimator $P(Y)\in\mathbb{R}^{n\times n}$ as following:
\begin{equation*}
 P_{ij}(Y)=\sum_{\alpha\in \textrm{NBW}(i,j)} \chi_\alpha(Y)
\end{equation*}
where $\textrm{NBW}_{\ell}(i,j)$ is the set of length-$\ell$ non-backtracking walk between $i$ and  $j$, $\chi_\alpha(Y)=\prod_{(u,v)\in\alpha} Y_{uv}^{t(\alpha,u,v)}$ where $t(\alpha,u,v)$ is the multiplicity of directed  hyperedge $(u,v)$ in $\alpha$.
\end{definition}
We prove in appendix \ref{NBWproof} that such estimator can be evaluated in nearly linear time if it achieves weak recovery 
\begin{theorem}[Evaluation of Non-backtracking walk estimator]\label{NBWevaluation}
In spiked matrix model defined in problem \ref{defWigner} , if $k$-step non-backtracking walk matrix $P(Y)\in \mathbb{R}^{n\times n}$ achieves weak recovery
\begin{equation*}
    \frac{\E \lprod P(Y),xx^\top\rprod}{n\left(\E \lVert P(Y)\rVert_F^2\right)^{1/2}}=\delta=\Omega(1)
\end{equation*}
then the span of top $\delta^{-O(1)}$ eigenvectors of $P(Y)$ can be evaluated in time  $O(n^2\log^{k+1} (n) \delta^{-O(1)} \exp(O(k)))$ if $\ell=O(\log n)$
\end{theorem}







==> broaderImpact.tex <==
\section*{Broader impact}
 We study an idealized mathematical model and provide theoretical analyses with only synthetic experimental validation. Therefore a direct impact on the society is out of reach. Potentially, since the problem we consider is closely related to stochastic block model, we speculate that our algorithm  could inspire the development of more robust and universal social network analysis. Further there is a chance that color coding method could point out new directions for sum-product evaluation in some types of neural network.
 
 Since the application area of the algorithm is still not clear, the positive and negative sides of algorithm really depend on what people are using it for.


==> contribution.tex <==




% \begin{definition}[non-Gaussian Wigner model]
% For non-Gaussian Wigner model, we have  $Y=\lambda xx^T+W$, where entries in $x\in \mathbb{R}^n$ and $W\in\mathbb{R}^{n\times n}$ are independent sampled with zero mean and $\E x_i^2=1$ and  $\E W_{ijk}^2=1$. We also assume $\E x_i^4=n^{o(1)}$.
% For recovery problem given matrix $Y$ we want to estimate the hidden vector $x$.
% \end{definition}
\subsection{Main contributions}
% For low degree algorithms, very sharp analysis is possible, which leads to very accurate computational threshold. Furthermore, for  tensor $Y$ sampled from planted distribution, since the algorithm only involves first and second moment of entries in $Y$, the guarantee of low degree algorithms can adapt to the distribution independent setting we consider in a black-box way.

First we observe that the self-avoiding walk estimator provided in  \cite{8104074} can actually solve the recovery problem in general Wigner model. 

\begin{theorem}[Guarantee in general spiked Wigner model]\label{Wigner}
When $\lambda\sqrt{n}=1+\Omega(1)$, we have polynomial time algorithm achieving weak recovery in general spiked Wigner model
\end{theorem}
The analysis in the original paper\cite{hopkins2018statistical} extends easily when planted vector $x$ is sampled from prior with zero mean and independent entries. Our technical contribution is to show that the guarantee extends to the case where $x$ is fixed vector with norm $\sqrt{n}$. Such guarantee is nontrivial since the universality of spectrum norm of random matrix requires bounded fourth moment while it is not required by our algorithm. 

% Although self-avoiding walk estimators can be evaluated in polynomial time, they are not practical, especially when $\lambda\sqrt{n}-1$ is small. Therefore we consider two algorithms as alternative. The first strategy is to truncate the entries with large amplitude. If the noise entries  are identically distributed then this strategy succeed when $\lambda>n^{-1/2}$ under mild assumption. However, it can fail drastically when we allow the entries to take different distribution. 

% The second strategy is to use non-backtracking walk as alternative. Such strategy works well in numerical experiments. But it's hard to prove the guarantee of such algorithms in general noise setting. 


% Compared to the guarantees in  \cite{Perry_2018}, a major advantage of low degree algorithms is that  it does not require knowledge about the underlying distribution of noise matrix. It's hard to apply their algorithm if the noise entries are independent but not identically distributed. 

% In general spiked tensor model. When the noise tensor is i.i.d  Gaussian, the same sharp  algorithm guarantees have been obtained in  \cite{hastings2019classical} while results sub-optimal by log-factors are known in \cite{hopkins2015tensor, Kikuchy}. 
In spiked tensor model, the guarantee of our algorithm extends to part of the sub-exponential region in the computational statistical gap.
\begin{theorem}[Guarantee in general spiked tensor model]\label{polyPCA}
  In the general spiked tensor model defined above, for $\gamma=0.001 n^{3/4}\lambda=\Omega(n^{-1/8+o(1)})$, we have $O(n^{\gamma^{-4}})$ time weak recovery algorithm and strong detection algorithm. When $\gamma=\omega(1)$, we have linear time strong detection algorithm and $n^{3+o(1)}$ time strong  recovery algorithm. 
\end{theorem}
  
%   $x^{\circ 3}$($x^{\circ 3}$ means the entry-wise power $3$ of vector $x$)
For recovery,the strategy we take is to find a vector $P(Y)\in\mathbb{R}^n$  whose entries are degree $v\log_{v\gamma^4} n$ polynomial where $v$ satisfies $v\gamma^4>1000$. It  achieves constant correlation with hidden vector
  \begin{equation*}
     \mathop{\E}\lprod P(Y),x\rprod=\Omega\left((\E\lVert   P(Y)\rVert    ^2)^{1/2}\left(\E \lVert   x\rVert^2\right)^{1/2}\right)
  \end{equation*}
  This imples weak recovery for spiked tensor model when $\gamma=\Omega(1)$. Further via a generalization of color coding method in  \cite{8104074}, we show that such polynomial can be evaluated in time $n^{O(\gamma^{-4})}$ for $\gamma=O(1)$. If $\gamma=\omega(1)$, then we have
    \begin{equation*}
     \mathop{\E}\lprod P(Y),x\rprod=(1-o(1))\left(\E\lVert   P(Y)\rVert^2\right)^{1/2}\left(\E \lVert   x\rVert^2\right)^{1/2}
  \end{equation*}
  which implies strong recovery. In this case we show that the polynomial vector $P(Y)$ can be evaluated in time $n^{3+o(1)}$
  
  For strong detection very similarly, when  $\gamma=\Omega(1)$, there is polynomial time strong detection algorithm by thresholding a scalar valued polynomial $P(Y)$ with maximum degree  $v\log_{v\gamma^4} n$  where $v$ satisfies $v\gamma^4>1$. By color coding method $P(Y)$ can be evaluated in time $O(n^{\gamma^{-4}})$. When $\gamma=\omega(1)$, thresholding a degree $2$ polynomial will be enough, which can be evaluated in linear time.  

We note that these results also extend to sub-exponential and quasi-polynomial regime by increasing degree of polynomial estimator. Such result matches the predicted lower bounds  \cite{kunisky2019notes} in part of the sub-exponential regime. However, it does not succeed until statistical threshold which is sub-optimal compared to previous results in case of Rademacher  \cite{bhattiprolu2016sumofsquares} or Gaussian noise distributions  \cite{hastings2019classical}.
% \begin{theorem}[Sub-exponential  algorithm for general spiked tensor model]\label{subPCA}
% In strong detection problem of general spiked tensor model,if we have $n^{3/2} \ell^{1/2} \lambda^2=\omega(1)$ and $\Gamma^2 n^{-1} \ell^2=o(1)$, then there is   $n^{O(\ell)}$ time  polynomial thresholding strong detection algorithm distinguishing the planted distribution and null distribution with probability $1-o(1)$.

% In recovery problem of general spiked tensor model, when
% $\ell=o(n^{1/2}\Gamma^{-1})$ and $\lambda^{-2}\ell^{-1/2} n^{-3/2}=o(1)$, there is estimation vector $P(Y)\in \mathbb{R}^n$ with each entry $P_i(Y)$ a degree $\ell\log n$ polynomial of entries in $Y$, achieving $1-o(1)$ correlation with  hidden vector $x$.  
% \begin{equation}
%     \frac{\E\lprod x,P(Y)\rprod}{\left(\E\lVert P(Y)\rVert^2\E\lVert x\rVert\right)^{1/2}}=1-o(1)
% \end{equation}
% and therefore gives a strong recovery algorithm.
% \end{theorem}

% The algorithm generalizes easily to partial observation case. Such tradeoff for boolean case(random 3-XOR) and bounded noise distribution have been known previously in [\cite{Barak2016},\cite{10.1145/3055399.3055417}].  The previous algorithms provided have additional log-factors.
% \begin{theorem}[partial observation recovery]\label{polysubPartial}
%     In general partially observation spiked tensor model, when $v=o(n^{1/2}\Gamma^{-1}\ell^{-1})$ and $\lambda^{2}v^{1/2}m n^{-3/2}=\omega(1)$,there is estimator $P_\Omega(Y)\in \mathbb{R}^n$ with each entry degree $O(v\log n)$ polynomial achieving $1-o(1)$ correlation with the hidden vector $x$,
% \begin{equation*}
%         \frac{\E[\lprod x,P_{\Omega}(Y)\rprod]}{\left(\E[\lVert P_{\Omega}(Y)\rVert^2]\E[\lVert x\rVert^2]\right)^{1/2}}=1-o(1)
% \end{equation*}
% Further $P_\Omega(Y)$ can be evaluated in $n^{O(v)}$ time.
% \end{theorem}

% \subsubsection{Lower bound results}
% The lower bound against low degree strong detection algorithms in spiked tensor model has been well studied before [\cite{kunisky2019notes,hopkins2018statistical}] and matches the guarantee of our algorithms above when $v=o(n^{1/2}\Gamma^{-1}\ell^{-1})$.  For random-3XOR, the lower bound results are also claimed in previous literature. Here we provide lower bound for partial spiked tensor model with Gaussian noise. 
% \begin{theorem}[Lower bound for partial observation with Gaussian noise]\label{lowerBound}
% In partially observed spiked tensor model: $Y_{ijk}=\lambda x_ix_jx_k+W_{ijk}$ for all $(i,j,k)\in\Omega$ with $\lambda<1$, if $x$ sampled from i.i.d Rademacher and $W_{ijk}$ i.i.d sampled from $N(0,1)$, then
% \begin{equation*}
%     \mathop{\textrm{max}}_{f(Y,\Omega)\in \textrm{poly}(Y,\Omega,\ell)}\frac{\E_{(Y,\Omega)\sim \mathbb{P}}f(Y,\Omega)}{\left(\E_{(Y,\Omega)\sim \mathbb{Q}} f^2(Y,\Omega)\right)^{1/2}}=O(1)
% \end{equation*}
% if and only if $\frac{\lambda^2 m}{n^{3/2}}\ell^{1/2}=O(1)$ and $m\lambda^4=O(1)$. Here $\text{poly}(Y,\Omega,\ell)$ means the polynomial space spanned by the multilinear monomials consisting of entries in $Y$ belonging to $\Omega$ and with degree smaller than $\ell$, i.e, for multi-hypergraph $\alpha \subseteq \Omega$(all hyperedges in $\alpha$ are contained in $\Omega$) with less than $\ell$ hyperedges, the corresponding polynomial basis is given by Hermite polynomial basis
% \begin{equation*}
%     \chi_\alpha(Y)=\prod_{(i,j,k)\in\alpha} h_{\alpha(i,j,k)}(Y_{ijk})
% \end{equation*}
% where $\alpha(i,j,k)$ is the multiplicity of hyperedge $(i,j,k)$ in hypergraph $\alpha$ and $h_{k}(y)$ is the degree-$k$ single variable normalized Hermite polynomial basis.
% \end{theorem}

% The only difference from random 3-XOR lies in that the low degree likelihood ratio  will still diverge if $m\lambda^4=\omega(1)$. Indeed, strong detection algorithm by thresholding  polynomial(not multilinear) exists in case of Gaussian noise if  $m\lambda^4=\omega(1)$, which is provided in appendix \ref{nonMultilinear}.





==> correlationPreservation.tex <==
\subsection{Strong recovery from 1-o(1) correlation}\label{StrongRecoveryFromCorrelation}
In this section, we show that if we have achieved $1-o(1)$ correlation under the framework of low degree algorithms, then strong recovery algorithm follows, i.e, we have unit norm estimator achieving $1-o(1)$ correlation with hidden vector with $1-o(1)$ probability. 

\subsubsection{Strong recovery from first moment correlation}
\begin{theorem}[Strong recovery from $1-o(1)$ correlation]
    Suppose we have $Y=f(x,W)$ where $x$ is sampled from i.i.d prior with
    \begin{equation*}
        \mathbb{E}x_i^2=1
    \end{equation*}
    and $W_{i_1i_2\ldots i_p}$ is i.i.d sampled from noise distribution.Suppose we have estimating vector $P(Y)\in \mathbb{R}^n$ achieving constant correlation with hidden vector $x$ 
    \begin{equation}
        \frac{\E\lprod P(Y),x\rprod}{\left(\mathbb{E}||P(Y)||^2 \mathbb{E} ||x||^2 \right)^{1/2}}=1-o(1)
    \end{equation}
    Further we assume that
    \begin{equation}
        \mathbb{E} x_i^4=n^{o(1)}
    \end{equation}
    (which is needed for the concentration of $\lVert x\rVert^2$),
    then we have following results
    \begin{itemize}
        \item[(a)] Estimation error
        \begin{equation}
        \mathbb{E} \left\lVert\frac{P(Y)}{\left(\mathbb{E} ||P(Y)||^{2}\right)^{1/2}}-\frac{x}{\left(\mathbb{E} ||x||^{2}\right)^{1/2}}\right\rVert=o(1)
        \end{equation}
        \item[(b)] Self-normalization
        \begin{equation*}
         \mathbb{P}\left(||P(Y)||=(1\pm o(1))\left(\mathbb{E} \lVert P(Y)\rVert^2\right)^{1/2}\right)=1-o(1)
        \end{equation*}
    \item[(c)] Strong recovery by normalized estimator
    \begin{equation*}
        \left\lprod\frac{P(Y)}{\lVert P(Y)\rVert},\frac{x}{\left(\mathbb{E}\lVert x\rVert^2\right)^{1/2}} \right\rprod=1-o(1)
    \end{equation*}
    with $1-o(1)$ probability
    \end{itemize}
\end{theorem}
\begin{proof}
First because 
    \begin{equation}
        \frac{\E\lprod P(Y),x\rprod}{\left(\mathbb{E}\lVert P(Y)\rVert^2 \mathbb{E} \lVert x\rVert^2 \right)^{1/2}}=1-o(1)
    \end{equation}
by equivalent transformation we have

\begin{align*}
    \left\lprod\frac{P(Y)}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}},\frac{x}{\left(\mathbb{E} \lVert x\rVert^2 \right)^{1/2}}\right\rprod  &=1-o(1)\\
    2-\mathbb{E}\left[\left\lVert \frac{P(Y)}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}-\frac{x}{\left(\mathbb{E} \lVert x\rVert^2 \right)^{1/2}}\right\rVert^2\right] &=2-o(1)\\
    \mathbb{E}\left[\left\lVert \frac{P(Y)}{\left(\mathbb{E}||P(Y)||^2\right)^{1/2}}-\frac{x}{\left(\mathbb{E} ||x||^2 \right)^{1/2}}\right\rVert^2\right] &=o(1)\\
\end{align*}
This proves the first statement. 

For the second statement, because $x$ is sampled from i.i.d prior, we have
\begin{equation*}
    \mathbb{P}\left(\lVert x\rVert^2=(1\pm o(1))\mathbb{E}\lVert
    x\rVert^2\right)=1-o(1)
\end{equation*}
Further from the above result we have
\begin{equation*}
    \E\left[\left(\left\lVert\frac{P(Y)}{\left(\E \lVert P(Y)\rVert^2\right)^{1/2}}
    \right\rVert -
 \left\lVert\frac{x}{\left(\E \lVert x\rVert^2\right)^{1/2}}
    \right\rVert  
    \right)^2\right]=o(1)
\end{equation*}
Therefore, 
\begin{equation*}
  \left\lVert\frac{P(Y)}{\left(\E \lVert P(Y)\rVert^2\right)^{1/2}}
    \right\rVert-
   \left\lVert\frac{x}{\left(\E \lVert x\rVert^2\right)^{1/2}}
    \right\rVert = o(1) 
\end{equation*}
with $1-o(1)$ probability. 
Combining these two arguments, we have
\begin{equation*}
    \frac{\lVert P(Y)\rVert^2}{\mathbb{E}\lVert P(Y)\rVert^2}=1-o(1)
\end{equation*}
with $1-o(1)$ probability. This prove the self-normalization property.

Finally, we want to prove the strong recovery achieved by normalized estimator. 
 We have
\begin{align*}
    \left\lVert\frac{P(Y)}{\lVert P(Y)\rVert}-\left(\frac{P(Y)}{\left(\mathbb{E}||P(Y)||^2\right)^{1/2}}\right)\right\rVert&=\left\lVert \frac{P(Y)}{\lVert P(Y)\rVert}\left(\frac{\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}-1\right)
    \right\rVert\\
    & = 1-\frac{\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}
    % & = 1-\frac{\E\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}
\end{align*}
Since we already have
\begin{equation*}
    \frac{\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}=1-o(1)
\end{equation*}
with $1-o(1)$ probability and
% and
%     \begin{equation*}
%         \frac{\E\lprod P(Y),x\rprod}{\left(\mathbb{E}\lVert P(Y)\rVert^2 \mathbb{E} \lVert x\rVert^2 \right)^{1/2}}=1-o(1)
%     \end{equation*}

%
% with $1-o(1)$ probability, and by Jensen's inequality
% \begin{equation*}
%     \mathbb{E} \lVert P(Y)\rVert\leq \left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}
% \end{equation*}
% Therefore, we have
% \begin{equation*}
%   \frac{\E\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}-1=o(1) 
% \end{equation*}
\begin{equation*}
    \left\lVert \frac{P(Y)}{\left(\mathbb{E}||P(Y)||^2\right)^{1/2}}-\frac{x}{\left(\mathbb{E} ||x||^2 \right)^{1/2}}\right\rVert =o(1)
\end{equation*}
with high probability.
Therefore by triangle inequality, we have
\begin{align*}
    \left\lVert \frac{P(Y)}{\lVert P(Y)\rVert}-\frac{x}{\left(\mathbb{E}\lVert x\rVert^2\right)^{1/2}}\right\rVert &\leq \left\lvert
    \frac{\lVert P(Y)\rVert}{\left(\mathbb{E}\lVert P(Y)\rVert^2\right)^{1/2}}-1\right\rvert \quad\large{+}\\ & 
    \left\lVert \frac{P(Y)}{\left(\mathbb{E}||P(Y)||^2\right)^{1/2}}-\frac{x}{\left(\mathbb{E} ||x||^2 \right)^{1/2}}\right\rVert
\end{align*}
As a result, we have 
\begin{equation*}
     \left\lVert \frac{P(Y)}{\lVert P(Y)\rVert}-\frac{x}{\left(\mathbb{E}\lVert x\rVert^2\right)^{1/2}}\right\rVert=o(1)
\end{equation*}
with $1-o(1)$ probability. Equivalently, we have
\begin{equation*}
    \left\lprod \frac{P(Y)}{\lVert P(Y)\rVert}, \frac{x}{\left(\mathbb{E}\lVert x\rVert^2\right)^{1/2}}\right\rprod=1-o(1)
\end{equation*}
with $1-o(1)$ probability.
\end{proof}
\subsubsection{Strong recovery from second moment correlation}
\begin{theorem}[Strong recovery from $1-o(1)$ correlation]
    Suppose we have $Y=f(x,W)$ where $x$ is sampled from i.i.d prior with
    $
        \mathbb{E}x_i^2=1
    $
    and $W_{i_1i_2\ldots i_p}$ is i.i.d sampled from noise distribution.Suppose we have symmetric estimator matrix $P(Y)\in \mathbb{R}^{n\times n}$ achieving constant correlation with hidden vector $x$ 
    \begin{equation}
        \frac{\E\lprod P(Y),x\rprod}{\left(\mathbb{E}||P(Y)||_F^2 \mathbb{E} ||xx^\top||_F^2 \right)^{1/2}}=1-o(1)
    \end{equation}
    Further we assume that
    \begin{equation}
        \mathbb{E} x_i^4=n^{o(1)}
    \end{equation}
    (which is needed for the concentration of $\lVert x\rVert^2$),
    then we have following results
    \begin{itemize}
        \item[(a)] estimation error
        \begin{equation}
        \mathbb{E} \left\lVert\frac{P(Y)}{\left(\mathbb{E} ||P(Y)||_F^{2}\right)^{1/2}}-\frac{xx^\top}{\left(\mathbb{E} ||x||^{4}\right)^{1/2}}\right\rVert^2=o(1)
        \end{equation}
        \item[(b)] self-normalization
        \begin{equation*}
         \mathbb{P}\left(||P(Y)||_F=(1\pm o(1))\left(\mathbb{E} \lVert P(Y)\rVert_F^2\right)^{1/2}\right)=1-o(1)
        \end{equation*}
    \item[(c)] strong recovery by normalized estimator: if we take the leading eigenvector of matrix $\xi=\frac{P(Y)}{\lVert P(Y)\rVert_F}$, then
    \begin{equation*}
        \left\lprod\frac{\xi}{\lVert \xi\rVert},\frac{x}{\lVert x\rVert} \right\rprod^2=1-o(1)
    \end{equation*}
    with $1-o(1)$ probability
    \end{itemize}
\end{theorem}

\begin{proof}
    For the first two properties, noting that
    \begin{equation*}
        \E \lVert x\rVert^4=(1+o(1)) \left(\E \lVert x\rVert^2\right)^2 
    \end{equation*}
    the proof is very similar to the vector case above. 
    
    For the third property, as in the vector case, we can derive that w.h.p
    \begin{equation*}
        \left\lprod \frac{P(Y)}{\lVert P(Y)\rVert_F}, \frac{xx^\top}{\left(\E\lVert x\rVert^4\right)^{1/2}}\right\rprod=1-o(1)
    \end{equation*}
    Because of Jensen's inequality and the concentration of $\lVert x\rVert^2$, we have
    \begin{equation*}
        \left\lprod \frac{P(Y)}{\lVert P(Y)\rVert_F}, \frac{xx^\top}{\lVert x\rVert^2}\right\rprod =1-o(1)
    \end{equation*}
    We consider the spectrum decomposition of $P^{\prime}(Y)=\frac{P(Y)}{\lVert P(Y)\rVert_F}$
    \begin{equation*}
        P^{\prime}(Y)=\sum_{\lambda=1}^n \lambda_i u_iu_i^\top
    \end{equation*}
    Then $\sum_{i=1}^n \lambda_i^2=1$ since $P^{\prime}(Y)$ has unit Frobenius norm. Therefore for unit vector $x^{\prime}=x/\lVert x\rVert$
    \begin{equation*}
        \sum_{i=1}^n\lambda_i(u_i^\top x^{\prime})^2=1-o(1)
    \end{equation*}
    with high probability. Since
    \begin{equation*}
        \sum_{i=1}^n \left(u_i^\top x^{\prime}\right)^2=1
    \end{equation*}
    therefore we have the leading eigenvalue $\lambda_1=1-o(1)$ w.h.p. Therefore, other eigenvalues are $o(1)$. As a result, 
    \begin{equation*}
        \sum_{i=2}^n \lambda_i \left(u_i^\top x^{\prime}\right)^2=o(1)
    \end{equation*}
    Therefore $\lambda_1 \left(\xi^\top x^{\prime}\right)^2=1-o(1)$ w.h.p, where $\xi$ is the leading eigenvector. This leads to the conclusion that $\left(\xi^\top x^{\prime}\right)^2=1-o(1)$ w.h.p, which proves the third property. 
\end{proof}

\subsubsection{Low degree algorithm for strong recovery}
In all, according to the above discussion, when we have vector low degree estimator $P(Y)\in \mathbb{R}^n$ achieving $1-o(1)$ correlation with the second moment of hidden vector $x$, 
    \begin{equation*}
    \frac{\E\lprod P(Y),x\rprod}{\left(\mathbb{E}||P(Y)||^2 \mathbb{E} ||x||^2 \right)^{1/2}}=1-o(1)
    \end{equation*}
Then we can simply normalize it $\hat{x}=\frac{P(Y)}{\lVert P(Y)\rVert}$ and we have strong recovery guarantee with high probability:
\begin{equation*}
    \lprod\hat{x}, \frac{x}{\lVert x\rVert}\rprod=1-o(1)
\end{equation*}


On the other hand, if we have matrix low degree estimator $P(Y)\in \mathbb{R}^{n\times n}$ achieving $1-o(1)$ correlation with $xx^\top$:
    \begin{equation*}
        \frac{\E\lprod P(Y),xx^\top\rprod}{\left(\mathbb{E}||P(Y)||_F^2 \mathbb{E} ||xx^\top||_F^2 \right)^{1/2}}=1-o(1)
    \end{equation*}
Then we can take the $\hat{x}$ as the leading eigenvector of $P(Y)/\lVert P(Y)\rVert$. Then we have w.h.p
\begin{equation*}
    \lprod\hat{x}, \frac{x}{\lVert x\rVert}\rprod^2=1-o(1)
\end{equation*}


==> polyAlgoTensorCompletion.tex <==

%Obsolete

% *************


% \section{Partial observation case}
% As defined before, in partial observation case we randomly observe a set of entries $\Omega=\{(i,j,k):i,j,k\in [n]\}$ in tensor $Y=\lambda x^{\otimes 3}+W$.  Then we can view $\Omega$ as a simple hypergraph. A natural idea for estimating $x\in \mathbb{R}^n$ is to use the sum of multilinear monomials corresponding to hypergraph $\alpha$ satisfying $\alpha\subseteq \Omega$.
% \begin{definition}[Recovery estimator in partial observation case]
%     In tensor completion given the set of locations defined above $\Omega=\{(i,j,k)\}$ and corresponding observation values $\{Y_{ijk}:(i,j,k)\in \Omega\}$, we select the following degree $(2\ell-1)v$ estimator $P_\Omega(Y)\in \mathbb{R}^n$ with $i$-th entry given by :
%     \begin{equation*}
%         P_{\Omega,i}(Y)=\sum_{\substack{\alpha\subseteq\Omega\\ \alpha \in S_{\ell,v,i}}} \chi_\alpha(Y)
%     \end{equation*}
%     where $S_{\ell,v,i}$ is the set of hypergraph   defined in the estimator of spiked tensor model while $\chi_\alpha(Y)=\prod_{(i,j,k)\in \alpha} Y_{ijk}$ is the Fourier basis corresponding to hypergraph $\alpha$. 
% \end{definition}
% Next we prove theorem \ref{polysubPartial} via analyzing guarantee of such estimator.
% % \begin{theorem}
% %     In general partially observation spiked tensor model, the above estimator $P(Y)\in \mathbb{R}^n$ achieves $1-o(1)$ correlation with the hidden vector $x$,
% % \begin{equation*}
% %         \frac{\E[x_iP_{i,\Omega}(Y)]}{\left(\E[P_{i,\Omega}(Y)^2]\right)^{1/2}}=1-o(1)
% % \end{equation*}
% % when $v=o(n^{1/2}\Gamma^{-1})$ and $\lambda^{2}v^{1/2}m n^{-3/2}=\omega(1)$ 
% % \end{theorem}
% \begin{proof}
 
%     For any hypergraph $\alpha$ with $k$ hyperedges, the probability that $\alpha\subseteq \Omega$ is given by $\left(\frac{m}{n^3}\right)^{k}$. Therefore
%     we have $$\E[x_iP_i(Y)]= \E_{\Omega} \sum_{\substack{\alpha\subseteq\Omega\\ \alpha\in S_{\ell,v,i}}} \lambda^{(2\ell-1) v}=\sum_{\alpha\in S_{\ell,v,i}} (m\lambda^2/n^3)^{(2\ell-1) v}$$ $$\E[P_i^2(Y)]=\E_{\Omega}\sum_{\substack{\alpha,\beta\subseteq\Omega\\ \alpha,\beta\in S_{\ell,v,i}\\ \lvert \alpha\cap\beta\rvert=k}} \lambda^{2(2\ell-1) v-2k} = \sum_{\substack{ \alpha,\beta\in S_{\ell,v,i}\\ \lvert \alpha\cap\beta\rvert=k}} (m\lambda^2/n^3)^{2(2\ell-1) v-2k}$$. Therefore  making variable change $m\lambda^2/n^3\to \bar{\lambda}^2$, this is equivalent to the correlation in spiked tensor model $Y=\bar{\lambda} x^{\otimes 3}+W$. The algorithm guarantee follows immediately from the corresponding guarantee in spiked tensor model 
% \end{proof}
% Further for constant $v$ we note that $P_\Omega(Y)$ can be evaluated in polynomial time via color coding method in the same way as in spiked tensor model, by viewing the  $Y$ as order-$3$ tensor with unobserved entries filled with $0$. This solves the strong recovery problem of partially observed spiked tensor model.

% By very similar argument, the strong detection algorithm by thresholding polynomial succeeds when $\ell v=o(n^{1/2}\Gamma^{-1/2})$ and $\lambda^{2}(\ell v)^{1/2}m n^{3/2}=\Omega(1)$.

% % \subsection{Lower bound for Gaussian noise case}
% % % \begin{definition}[Tensor completion with Gaussian noise]
% % % We want to distinguish two distributions below with $1-o(1)$ probability
% % % \begin{itemize}
% % %     \item planted distribution $\mathbb{P}$:We sample a set $\Omega=\{(i,j,k)\}$ such that for each $(i,j,k)\in [n]^{\otimes 3}$, $(i,j,k)\in\Omega$ with probability  $m/n^3$. Then $\forall (i,j,k)\in \Omega$, we have
% % %     $Y_{ijk}=\lambda x_ix_jx_k+W_{ijk}$
% % % where $x\in \{\pm 1\}^n$ is sampled from i.i.d Rademacher distribution  and $W\in \mathbb{R}^{n\times n\times n}$ with i.i.d entries $W_{ijk}\in N(0,1)$.
% % % \item null distribution $\mathbb{Q}$: $\Omega$ sampled in the same way while $Y_{ijk}$ i.i.d sampled from $N(0,1)$
% % % \end{itemize}
% % % We can think of $Y$ as a $n\times n\times n$ tensor by filling the unobserved entries with $0$
% % % \end{definition}
% % % \begin{theorem}[Lower bound for tensor completion with Gaussian noise]
% % % For the above detection problem with $\lambda<1$,we have
% % % \begin{equation}
% % %     \mathop{\textrm{max}}_{f(Y,\Omega)\in \textrm{poly}(Y,\Omega,\ell)}\frac{\E_{(Y,\Omega)\sim \mathbb{P}}f(Y,\Omega)}{\left(\E_{(Y,\Omega)\sim \mathbb{Q}} f^2(Y,\Omega)\right)^{1/2}}=O(1)
% % % \end{equation}
% % % if and only if $\frac{\lambda^2 m}{n^{3/2}}\ell^{1/2}=O(1)$. Here $\text{poly}(Y,\Omega,\ell)$ means the polynomial space spanned by the multilinear monomials consisting of entries in $Y$ belonging to $\Omega$ and with degree smaller than $\ell$, i.e, for multi-hypergraph $\alpha \subseteq \Omega$(all hyperedges in $\alpha$ are contained in $\Omega$) with less than $\ell$ hyperedges, the corresponding polynomial basis is given by Hermite polynomial basis
% % % \begin{equation*}
% % %     \chi_\alpha(Y)=\prod_{(i,j,k)\in\alpha} h_{\alpha(i,j,k)}(Y_{ijk})
% % % \end{equation*}
% % % where $\alpha(i,j,k)$ is the multiplicity of hyperedge $(i,j,k)$ in hypergraph $\alpha$ and $h_{\alpha(i,j,k)}(Y_{ijk})$ is the degree-$k$ single variable normalized Hermite polynomial basis.
% % % \end{theorem}
% % We prove the lower bound result theorem \ref{lowerBound}
% % \begin{proof}
% % With the same derivation as in the Boolean case, we have
% % \begin{equation*}
% %     \mathop{\textrm{max}}_{f(Y,\Omega)\in \textrm{poly}(Y,\Omega,\ell)}\frac{\E_{(Y,\Omega)\sim \mathbb{P}}f(Y,\Omega)}{\left(\E_{(Y,\Omega)\sim \mathbb{Q}} f^2(Y,\Omega)\right)^{1/2}}
% %     =\mathop{\mathbb{E}}_\Omega\sum_{\substack{\alpha\subseteq\Omega\\ |\alpha|\leq \ell}} \hat{\mu}_\alpha^2=\sum_{\substack{|\alpha|\leq \ell}}  \left(\frac{m}{n^3}\right)^{D_\alpha} \lambda^{2\ell_\alpha}
% % \end{equation*}
% % where we denote the number of distinct hyperedges in $\alpha$ as $D_\alpha$ and number of hyperedges in $\alpha$ as $\ell_\alpha$.
% % Obviously we have $D_\alpha\leq \ell_\alpha$

% % % To tackle with this summation, we note that for each even degree multi-hypergraph $\alpha$, it can be obtained by adding edges to a even degree simple hypergraph $\alpha^{\prime}$. $\alpha^{\prime}$ can be obtained from $\alpha$ by maintaining all hyperedges with even multiplicity and deleting all hyperedges with odd multiplicity. 

% % We note that each even degree multi-hypergraph $G$ can be generated by the following process
% % \begin{itemize}
% %     \item choose a pair of even degree simple hypergraph with no intersecting edges $(\alpha,\beta)$
% %     \item Obtain multi-hypergraph $\alpha^{\prime}$ from $\alpha$ by adding even  multiplicity to each hyperedge contained in $\alpha$. Obtain multi-hypergraph  $\beta^{\prime}$ from $\beta$ by adding odd multiplicity to each hyperedge contained in $\beta$.
% %     \item $G$ given by $\alpha^{\prime}\cup \beta^{\prime}$
% % \end{itemize}
% % We denote the number of hyperedges in $\alpha,\beta$ as $\ell_\alpha,\ell_\beta$. Further, we denote that $i$-th hyperedge in simple hypergraph $\alpha$ has multiplicity $1+t_i$ in hypergraph $G$ and $i$th hyperedge in simple hypergraph  $\beta$ has multiplicity $2+t^{\prime}_i$ in $G$. Then we have $\forall i~ t_i,t^{\prime}_i\geq 0$. Therefore the above summation is upper bounded by
% % \begin{align*}
% %      &\sum_{\substack{\alpha\subseteq\Omega\\ |\alpha|\leq \ell \\\alpha\text{ is simple}}}
% %     \sum_{\substack{\beta\subseteq\Omega\\ |\beta|\leq \ell \\\beta\text{ is simple}\\\beta\cap\alpha=\emptyset}}
% %         \left(\frac{m}{n^3}\right)^{\ell_\beta+\ell_\alpha} \left(\sum_{ t_1,t_2,\ldots,t_{\ell_\alpha}}\lambda^{2(\ell_\alpha+\sum_{i=1}^{\ell_\alpha} t_i)}\right)
% %     \left(\sum_{ t_1,t_2,\ldots,t_{\ell_\beta}} \lambda^{2\left(\sum_{i=1}^{\ell_\beta}(2+t^{\prime}_i)\right)}
% %     \right)
% %     \\
% %     =&  \sum_{\substack{\alpha\subseteq\Omega\\ |\alpha|\leq \ell \\\alpha\text{ is simple}}}
% %     \sum_{\substack{\beta\subseteq\Omega\\ |\beta|\leq \ell \\\beta\text{ is simple}\\
% %     \beta\cap\alpha=\emptyset}} 
% %     \left(\frac{m}{n^3}\right)^{\ell_\beta+\ell_\alpha} 
% %     \lambda^{2\ell_\alpha}\left(\frac{\lambda^2}{\lambda^2-1}\right)^{2\ell_\alpha} \lambda^{4\ell_\beta}\left(\frac{\lambda^2}{\lambda^2-1}\right)^{2\ell_\beta}\\
% %     \leq & \sum_{\ell_\alpha=0}^{\ell} \sum_{\ell_\beta=0}^{\ell}
% %     \left(\frac{m}{n^3}\right)^{\ell_\beta+\ell_\alpha} 
% %     \lambda^{2\ell_\alpha}\left(\frac{\lambda^2}{\lambda^2-1}\right)^{2\ell_\alpha} \lambda^{4\ell_\beta}\left(\frac{\lambda^2}{\lambda^2-1}\right)^{2\ell_\beta} n^{3\ell_\beta} {n\choose 3\ell/2}  \frac{(3\ell_\alpha)^{3\ell_\alpha}}{\ell_\alpha!}\\
% %      =& \sum_{\ell_\alpha}\sum_{\ell_\beta} \left(c_1m \lambda^2 n^{-3/2}\ell_\alpha^{1/2}\right)^{\ell_\alpha} \left(c_2m\lambda^4\right)^{\ell_\beta}
% % %   \sum_{\substack{\alpha\subseteq\Omega\\ |\alpha|\leq \ell \\\alpha\text{ is simple}}} \left(\frac{m}{n^3}\right)^{\ell_\alpha} \sum_{ t_1,t_2,\ldots,t_{\ell_\alpha}}\lambda^{2(\ell_\alpha+\sum_{i=1}^{\ell_\alpha} t_i)}\leq  \sum_{\substack{\alpha\subseteq\Omega\\ |\alpha|\leq \ell \\\alpha\text{ is simple}}}  \left(\frac{m}{n^3}\right)^{\ell_\alpha}\lambda^{2\ell_\alpha} \left(1-\frac{1}{\lambda^2}\right)
% % \end{align*}
% % where $c_1$ and $c_2$ are constants. Therefore if $\frac{m}{n^3}\lambda^2 n^{3/2}\ell_\alpha^{1/2}=o(1)$ and $m\lambda^4=o(1)$, then the low degree likelihood ratio is bounded. Further when  $m\lambda^4=\omega(1)$ or $\frac{m}{n^3}\lambda^2 n^{3/2}\ell_\alpha^{1/2}=\omega(1)$, the low degree likelihood ratio is unbounded. (We will give algorithm in this case in appendix.)
% % \end{proof}

